IC-Portrait: In-Context Matching for View-Consistent Personalized Portrait

Existing diffusion models show great potential for identity-preserving generation. However, personalized portrait generation remains challenging due to the diversity in user profiles, including variations in appearance and lighting conditions. To address these challenges, we propose IC-Portrait, a novel framework designed to accurately encode individual identities for personalized portrait generation. Our key insight is that pre-trained diffusion models are fast learners (e.g.,100 ~ 200 steps) for in-context dense correspondence matching, which motivates the two major designs of our IC-Portrait framework. Specifically, we reformulate portrait generation into two sub-tasks: 1) Lighting-Aware Stitching: we find that masking a high proportion of the input image, e.g., 80%, yields a highly effective self-supervisory representation learning of reference image lighting. 2) View-Consistent Adaptation: we leverage a synthetic view-consistent profile dataset to learn the in-context correspondence. The reference profile can then be warped into arbitrary poses for strong spatial-aligned view conditioning. Coupling these two designs by simply concatenating latents to form ControlNet-like supervision and modeling, enables us to significantly enhance the identity preservation fidelity and stability. Extensive evaluations demonstrate that IC-Portrait consistently outperforms existing state-of-the-art methods both quantitatively and qualitatively, with particularly notable improvements in visual qualities. Furthermore, IC-Portrait even demonstrates 3D-aware relighting capabilities.

==> Method.tex <==
% Some commands used in this file
\newcommand{\package}{\emph}

\section{Method}


\subsection{Motivation}

In the domain of portrait generation, existing methods such as IP-Adapter~\cite{IP-Adapter}, FastComposer~\cite{FastComposer}, and Photomaker~\cite{photomaker} exhibit certain limitations, which have spurred the development of our proposed approach. Embedding-based one-shot methods, designed to handle identity representation, face challenges. These methods rely on extracted embeddings of fixed dimensions from the model. These however fail to capture the intricate intricate nature of the human identity in portraits, and only capture a restricted amount of information. Consequently, the portrait results they produce often have a low resemblance. For instance, when generating a portrait of a particular individual, these methods might fail to precisely capture the unique facial contours, expressions, and other minute details that define the person's identity.


On the other hand, Dreambooth-like fine-tuning methods like Lora~\cite{Lora}, Dreambooth~\cite{Dreambooth}, and Easyphoto~\cite{easyphoto} attempt to learn the accurate identity from user profiles that are inherently inconsistent. As depicted in Fig. \ref{fig:diverse}, various elements such as diverse expressions, makeup, and lighting conditions significantly affect the identity representations. When endeavoring to train a customized model using only a few highly diverse user profiles, it becomes almost impossible to accurately represent the user's true identity. These methods usually yield only a rough approximation. For example, if a user supplies a collection of photos with varying lighting and expressions, the model may have difficulty generalizing and precisely depicting the user's core identity.


To further elucidate this issue, consider the example in Fig. \ref{fig:relight} with Taylor Swift. The embedding method generates results that are only approximately similar to the original, and essential details are lost during the process. This prompts us to question the traditional approach and explore alternative strategies. What if we could directly replicate the face from the subject's profile, as in the case of Taylor Swift? By doing so, we can then utilize reposing techniques, which are part of the novel-view synthesis process like DiffPortrait3d~\cite{DiffPortrait3d} and EG3D~\cite{EG3D}, to align the face accurately. Additionally, applying portrait relighting methods such as Lite2Relight~\cite{lite2relight}, DiffPortrait3d~\cite{DiffPortrait3d}, and LumiGAN~\cite{LumiGAN} can help make the copied face harmonious with the style reference. This novel concept forms the basis of our pipeline design, which involves splitting the portrait generation process into two distinct yet interconnected tasks: novel view synthesis and relightable stitching. Here we define stitching as a nearly copy-paste process.

Through this decomposition, we strive to overcome the limitations of current methods and offer a more precise and detailed portrait generation solution. By isolating and addressing the challenges related to identity preservation and style adaptation separately, we enhance the overall quality and fidelity of the generated portraits. We meticulously engineer each step of the process, from data handling to model training and inference. IC-Portrait is crafted to handle the subtleties that previous approaches overlooked, ensuring that the generated portraits not only capture the essence of the subject's identity but also blend seamlessly with the desired artistic style, presenting a final output that is both recognizable and aesthetically pleasing, thus meeting the high standards required in diverse applications such as professional photography, digital art, and social media profile customization.





\begin{figure}[thb]
  \centering
   \includegraphics[width=0.9\linewidth]{images/relight.jpg}
   \caption{We demonstrate the idea of copy-paste-relight. Conventional methods use an ID encoder to extract the embedding (``ID prompt"),but it may lose details of the ref ID. We plan to use a brute-force copy-paste and harmonize the pasted result, as in `Relight Fuse". The results here are not perfect, only for demonstration.}
   \label{fig:relight}
\end{figure}



\subsection{Data Synthesis}
%How to write this section: introduce the multi-view data generation process as given in Fig.~\ref{fig:multi-view}

The generation of multi-view data, as illustrated in Fig. \ref{fig:multi-view}, is a crucial step in our methodology. The process commences with the employment of SDXL, a powerful tool for generating human images. By randomly selecting celebrity names, we can obtain a diverse set of initial images that capture a wide range of human features and expressions following the procedures given in \cite{CelebBasis}. These images serve as the cornerstone for our data synthesis process.


Once the initial images are generated, they are reprojected into the latent space using a technique described in \citet{Single-Image}. This technique trains an encoder to map images to corresponding EG3D~\cite{EG3D} tri-planes and re-renders novel-views. This enables us to create multiple views of the same subject, thereby enriching our dataset with different perspectives. The diversity in views offers valuable information about the subject's appearance from various angles, which is essential for training models that need to handle different poses and orientations.

The above process enables us to generate pairs of multi-view images. We then randomly select from a pair of left/right images, one to act as the image reference. This random selection ensures that our dataset encompasses a wide variety of reference images, reducing bias and increasing the generalizability of our model. In the next step, we randomly drop the pixels in the other image, as shown in Fig. \ref{fig:pipeline} (left). This pixel-dropping process is a meticulously designed step to construct the control condition. By introducing this variability in pixel information, we can simulate different levels of light preservation and train our model to handle the identity-lighting trade-off. For example, when a larger percentage of pixels is dropped, the model has to rely more on the remaining information to maintain the identity while adjusting for the change in lighting. This helps enhance its robustness and adaptability in real-world applications.

\subsection{ID-ReferenNet}
%How to write this section: Introduce pixel sampling technique,inspired by mased autoencoders (MAE) pretraining. Checkerboard sampling has only uniform sampling grid and easily result in over-smooth results. We concatenate sampled pixel with the profile image with the synthetic multi-view data to construct the condition for ID-ReferenceNet training.
After creating our multi-view synthetic dataset, we can train our ID-ReferenceNet, which is a crucial component of IC-Portrait. The ID-ReferenceNet is constructed in the ControlNet~\cite{controlnet} style, but unlike traditional single input ControlNet, it has dual conditions of identity image reference and sparse pixels condition. Through this design, we are able to separate the identity from the lighting in the style reference image.


The ID-ReferenNet is a key part of our system, and its design is inspired by the principles of masked autoencoders (MAE)~\cite{MAE} pretraining. Pixel sampling plays a vital role in this context. Traditional sampling techniques, such as checkerboard sampling, have limitations. Checkerboard sampling, with its uniform sampling grid, often leads to overly-smooth results. This is because it fails to introduce complex spatial variations in the image, causing trivial convergence during the training process.


To address this issue, we introduce a more advanced pixel sampling technique. We concatenate the sampled pixels in the width dimension,$H\times 2W \times 3$, with the profile image from the synthetic multi-view data. This concatenation process forms a diverse set of dual-condition inputs for training the ID-ReferenceNet.

By incorporating the multi-view data, we provide the network with a comprehensive understanding of the subject's appearance from different perspectives. This combination of data sources and sampling techniques equips the ID-ReferenceNet with the ability to accurately represent and transfer identity information while preserving the given low-level lighting information during the portrait generation process.

Given a sampled view pair $z$ and $z'$  we get the input condition $c_f$ as:
\begin{equation}
    c_f={F}(z,0\sim n)\textcircled{c}z',
\end{equation} where ${F}(\cdot,n)$ means uniformly sample $n\%$ pixels in the image, and $\textcircled{c}$ means spatial width-wise concatenation. Here, we use $0\sim n$ to represent that we uniformly pick a value in the range $(0,n)$. Then we simply get the input data $z_0$ as:
\begin{equation}
    z_0=z\textcircled{c}z'.
\end{equation}
Given time step $t$ and we use $z'$ as CLIP~\cite{CLIP} image embedding prompt (remove text prompt), image diffusion algorithms learn a network (UNet) $\epsilon_\theta$ to predict the noise added to $z_t$ with:
\begin{equation}
\mathcal{L}=\mathbb{E}_{z_0,t,z',c_f,\epsilon\sim\mathcal{N}(0,1)}\left[ \lVert\epsilon - \epsilon_\theta(z_t,t,z') \rVert_2 \right].
\end{equation}
This equation $\mathcal{L}$ is the learning objective of training the ID-ReferenceNet in ControlNet~\cite{controlnet} Fashion. Recent practices such as DiffPortrait3d~\cite{DiffPortrait3d} and IDM-VTON~\cite{IDM-VTON} use reference in direct self-attention injection which is surely more effective but can lose generalizability with customized model.


\begin{figure*}[thb]
  \centering
   \includegraphics[width=0.9\linewidth]{images/pipeline.jpg}
   \caption{Here we present the pipeline of our method. IC-Portrait consists of two phases: 1) Cross-profile Customization. In this phase, a user-specific model is fine-tuned with user photo profiles. We remove the text prompt and use the CLIP image embedding extracted from a random user profile. 2) Dual Condition Inference. This phase applies our dual condition ID-ReferenceNet, which transfers the reference ID to our target image while maintaining low-level lighting information through pixel sampling. The reference profile and the sampled pixels are concatenated horizontally and fed into a ControlNet-style model. In this model, the features of the ReferenceNet are added to the customized UNet.}
   \label{fig:pipeline}
\end{figure*}

\subsection{Cross-profile Customization}
We aim to combine the benefits of Dreambooth fine-tuning, which permits learning specific identities from limited data, and the embedding method, which offers a broader feature representation, during the cross-profile customization phase.

Our objective is to fine-tune a user-specific model using user photo profiles. Dreambooth fine-tuning enables a personalized adaptation to each user's unique identity within the portrait, yet it may encounter overfitting or struggle to fully capture the diversity of the user's photos. While Dreambooth focuses on specific identities, the embedding method provides a more general feature representation but lacks precision in capturing individual identities. By integrating these two approaches, we seek to harness the strengths of each and mitigate the inherent trade-offs.

In our cross-profile customization phase, we deviate from the conventional approach. Typically, models rely on text prompts, such as “A [V] woman,” to guide the generation process. However, we acknowledge the limitations of such text-based prompts, especially when dealing with the complexity of user-specific portraits. Instead, we discard the text prompt and concentrate on the CLIP image embedding extracted from a random user profile. This embedding contains valuable visual information that better captures the unique characteristics of the user. Consequently, the customized model learns a profile-specific identity rather than a general ID representation.


To stabilize the customization process, we implement a non-trivial design choice: randomly pairing the image embedding profile with a noisy profile training image. This random pairing serves multiple purposes. First, it averts the simplistic copy-pasting of the user's image, which could lead to overfitting and poor generalization. By introducing randomness, the model is compelled to learn more generalizable features that are not solely reliant on the specific image. Second, this approach helps decouple lighting conditions. Since the noisy profile image may have different lighting compared to the user's original profile, the model learns to manage lighting variations. For example, if the original profile has soft lighting and the noisy profile has harsh lighting, the model can learn to adjust and generate portraits that appear consistent under different lighting scenarios, enhancing its performance in generating portraits under diverse lighting conditions.

% \begin{algorithm}
% 	\caption{Single-stage Dual Condition Inference}
% 	\label{alg:inference}
% 	\KwIn{Selected User Profile: $p$, Style Reference Image: $s$, Denoising Strength: $\delta$, ID Embedding Strength:$\gamma$, Pixel Sampling Ratio:$r$, Denosing\_steps: $S$.}
% 	\KwOut{Generated image $\widetilde{x}_0$.}
%         $e_{profile}=CLIP(p)$;\\
%         % $T \leftarrow N * \alpha$ \\
%         % $x_s = F(x_0, T)$ \\
%         $T'=T\delta$;\\
%         %
%         $T_{list}=[T',...,1]$, $len(T_{list})=S$; \\
%         %
%         $\epsilon \sim \mathcal{N}(\textbf{0},\textbf{I})$;\\
%         %
%         $\widetilde{x}_{T'} = \sqrt{\alpha_{T'}}s \textcircled{c} p + \sqrt{(1 - \alpha_{T'})}\epsilon $.\\
%         % Initialize $c$ to zero 

%         \For{$t=T_{list}[0],...,T_{list}[S-1]$}{
            
%             $\widetilde{x}'_{t-1} = \sqrt{\alpha_{t-1}}\left( \frac{x_t-\sqrt{1-\alpha_t}\epsilon_\theta^{t}(\left \widetilde{x}_t, {F}(s,r) \textcircled{c} p,e_{profile} \right)}{\sqrt{\alpha_t}} \right) + \sqrt{1 - \alpha_{t-1}-\sigma_t^2} \cdot \\ \qquad\quad \epsilon_\theta^{t}(\widetilde{x}_t, {F}(s,r) \textcircled{c} p,e_{profile});$
            
%             % $x'_t = B(x_s, s)$

        
%             $\epsilon \sim \mathcal{N}(\textbf{0},\textbf{I})$ if $t > 1$, else \epsilon=\textbf{0};\\
%             %
%             $s_{t-1} = \sqrt{\alpha_{t-1}}s$ + \sqrt{(1 - \alpha_{t
%             -1})}\epsilon;\\
%             $\widetilde{x}_{t-1} = \widetilde{x}'_{t-1} \odot (1 - m_{non\_face}) + m_{non\_face} \odot s_{t}.$
%             %
%         }
%         \Return $\widetilde{x}_0$
        
% \end{algorithm}

\subsection{Iterative Dual Condition Inference}
The dual condition inference phase is a vital part of our IC-Portrait system. In this phase, our dual-condition ID-ReferenceNet is applied to achieve accurate and detailed portrait generation. The primary function of this network is to transfer the reference ID to the target image in the form of self-attention reference while maintaining low-level lighting information, accomplished through pixel sampling, which has been carefully designed and integrated into the process.
The reference profile and the sampled pixels are concatenated horizontally as aforementioned in Algorithm~\ref{alg:inference} 


Within this model, the features of the ReferenceNet are incorporated into the customized UNet. This integration allows for a seamless combination of the identity-related information from the ReferenceNet with the generative capabilities of the UNet. 

This harmonious cooperation enables the model to generate portraits that accurately represent the reference ID while maintaining the integrity of the lighting and other visual details. For instance, the model can preserve the natural shadows and highlights on the face while ensuring the face structure and features match the reference ID, resulting in high-quality and visually appealing portrait images.

Specifically, we implement our dual condition inference as an iterative process where we gradually transfer the reference style into the target identity. By adding noise using the diffusion forward process as proposed in DDPM~\cite{DDPM}, we can control the noise level to avoid corrupting too much information provided by the style reference image. If we attempt to generate the identity in a single pass, it may lose the low-level features in the style reference such as JPEG compression cues or some image degradations. Generating a hyper-resolution face with a low-quality background and body is visually inconsistent.

Here we present the single-stage inference details in Algorithm \ref{alg:inference}. We first extract the embedding from the profile image to replace the text embedding. This embedding is fed into UNet and ID-ReferenceNet and influences the generating process within the cross-attention mechanism. Then, we combine the profile image with the pixel-sampled style reference as the dual condition input for the ID-ReferenceNet. We also utilize an inpainting technique which restores the known area in the latent space.


With the single-stage inference, we construct the iterative inference paradigm of IC-Portrait. We experiment with several design choices: few steps but larger strengths and more steps but smaller strengths. We discover that smaller strengths but more iterating steps lead to better ID transfer and consistent generation. We use 3 iterations by using the result from the previous pass as the input for the next generation with denoising strengths  for each iteration. The rationale behind this choice is that with smaller strengths in each iteration, the model can make more gradual and accurate adjustments to the image, progressively converging to a superior result that preserves both the identity and the style details.

    

